Co-occurrence Based Texture Synthesis

As image generation techniques mature, there is a growing interest in explainable representations that are easy to understand and intuitive to manipulate. In this work, we turn to co-occurrence statistics, which have long been used for texture analysis, to learn a controllable texture synthesis model. We propose a fully convolutional generative adversarial network, conditioned locally on co-occurrence statistics, to generate arbitrarily large images while having local, interpretable control over the texture appearance. To encourage fidelity to the input condition, we introduce a novel differentiable co-occurrence loss that is integrated seamlessly into our framework in an end-to-end fashion. We demonstrate that our solution offers a stable, intuitive and interpretable latent representation for texture synthesis, which can be used to generate a smooth texture morph between different textures. We further show an interactive texture tool that allows a user to adjust local characteristics of the synthesized texture image using the co-occurrence values directly.

==> figures/editing/editing.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=1.0\textwidth]{figures/editing/editing.png}
\caption{{\bfseries Interactive co-occurrence editing.} With our representation, a user can locally adjust the generated image by editing its corresponding co-occurrence matrix. %In our interactive system, users can select a bin in the matrix to modify. 
In the center, we illustrate the initial result and two selected regions and their co-occurrence matrices. 
%
We demonstrate the results obtained by multiplying a selected bin with an increasing factor to the left (editing the co-occurrence matrix inside the purple box) and to the right (editing the co-occurrence matrix inside the blue box). 
%In the middle row we illustrate representative samples conditioned on co-occurrences, obtained by multiplying a selected bin with an increasing factor. The top row and bottom row correspond to editing the co-occurrence of the top left bottom right regions, respectively.
}
\label{fig:interactive}
\end{center}
\end{figure*}
